Self-supervised video pretraining yields robust and more human-aligned visual representations

Humans learn powerful representations of objects and scenes by observing how they evolve over time. Yet, outside of specific tasks that require explicit temporal understanding, static image pretraining remains the dominant paradigm for learning visual foundation models. We question this mismatch, and ask whether video pretraining can yield visual representations that bear the hallmarks of human perception: generalisation across tasks, robustness to perturbations, and consistency with human judgements. To that end we propose a novel procedure for curating videos, and develop a contrastive framework which learns from the complex transformations therein. This simple paradigm for distilling knowledge from videos, called VITO, yields general representations that far outperform prior video pretraining methods on image understanding tasks, and image pretraining methods on video understanding tasks. Moreover, VITO representations are significantly more robust to natural and synthetic deformations than image-, video-, and adversarially-trained ones. Finally, VITO's predictions are strongly aligned with human judgements, surpassing models that were specifically trained for that purpose. Together, these results suggest that video pretraining could be a simple way of learning unified, robust, and human-aligned representations of the visual world.

==> tables/NIGHTS_table.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}

\begin{table*}[ht]

\small\centering
\begin{tabularx}{\linewidth}{l *{5}{Y}}
              Image type & VITO (R-50) & CLIP (VIT-B/32) & DINO (VIT-B/16) & MAE (VIT-H/14) & OpenCLIP (VIT-B/32) \\ 

\midrule
\vspace{-0.5em}  \\

Non-ImageNet Images & 86.5 & 82.1 & 89.5 & 83.8 & 87.6 \\
%ImageNet Images & 85.3 & 83.8 & 90.6 & 83.2 & 86.7 \\
\end{tabularx}
\label{tab:nights}
\caption{2AFC Alignment Score on perceptual similarity for the NIGHTS dataset}
\end{table*}

==> tables/geirhos-ablate.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}

\begin{table*}[ht]

\small\centering
\begin{tabularx}{\linewidth}{l *{4}{Y}}
              Method & Dataset & accuracy diff. $\downarrow$ & obs. consistency $\uparrow$ & ceiled error consistency $\uparrow$ \\

\midrule
\vspace{-0.5em}  \\
\multicolumn{2}{l}{\textit{VITO and Ablations}}
 \\
\rowcolor{DnCBG} VITO & VideoNet &                       \textbf{0.157} &                       \textbf{0.564} &                        \textbf{0.422}  \\
VITO & AudioSet &                       0.160 &                       0.557 &                        0.401  \\
VITO (w/o attn) & VideoNet &                       0.169 &                       0.554 &                        0.390  \\
VITO (1scale) & VideoNet &                       0.158 &                       0.553 &                        0.368  \\
VITO (1scale w/o attn) &  VideoNet &                     0.188 &                       0.533 &                        0.359  \\
VITO (spatial) & VideoNet &                      0.175 &                       0.533 &                        0.323  \\
 MoCLR &     VideoNet &                   0.241 &                       0.475 &                        0.224  \\
\\
\multicolumn{2}{l}{\textit{Prior work:}} \\
CLIP &  OpenAI-400M &            \textbf{0.108} &             \textbf{0.612} &              \textbf{0.482}  \\


L2 Robust 1.0  & ImageNet &                      0.178 &                       0.534 &                        0.389  \\



               MoCLR \cite{tian2019contrastive} & ImageNet &                      0.190 &                       0.536 &                        0.335  \\
                StyleTransfer &  SIN + ImageNet &                     0.203 &                       0.527 &                        0.330  \\
                 Supervised & ImageNet &                       0.215 &                       0.511 &                        0.329  \\

       
                       DINO \cite{caron2020unsupervised} & ImageNet &                       0.236 &                       0.504 &                        0.291  \\

               VINCE \cite{gordon2020watching} & R2V2 &                      0.210 &                       0.501 &                        0.269 \\

               CycleCon \cite{wu2021contrastive} &   R2V2 &                    0.237 &                       0.484 &                        0.258  \\
                 R3M \cite{nair2022r3m} &   Ego-4D &                     0.392 &                       0.359 &                        0.054  \\
                 VFS \cite{xu2021rethinking} & K-400 &                      0.394 &                       0.354 &                        0.049  \\
\end{tabularx}
\vspace{1em}
\caption{Accuracy difference and consistency with human judgments on stimuli for recognition/discrimination of shape-biased stimuli. We now provide extensive ablations with all aspects of VITO and against other strong image-models trained on video datasets. We also include CLIP for comparison which outperforms VITO but is trained on an order of magnitude larger dataset than all other methods. }
\label{tab:shapebias}
\vspace{-1em}
\end{table*}

==> tables/robustness.tex <==

\begin{table}[t]
% \vspace{-1.em}
\vspace{1.em}
\small
\centering
\begin{tabularx}{\columnwidth}{l *{4}{Y}}

% & & & \multicolumn{2}{c}{Semantic segmentation} \\
% \cmidrule(lr){4-5}
Method & Pretraining Dataset  & ImageNet-Vid-Robust (pm0/pm10) & ImageNet-A  \\
\midrule
\vspace{-0.9em} \\
Supervised & ImageNet & 67.7 ~ / ~ 52.4 & 2.2 \\
MoCLR & ImageNet &  64.7 ~ / ~ 50.0 & 3.7  \\ %& 27.5 & 28.9  \\
\rowcolor{DnCBG} \ours  & VideoNet  & \textbf{70.6} ~ / ~ \textbf{57.2} &  \textbf{5.4}  \\ %textbf{29.5} & \textbf{30.6} \\


\end{tabularx}

\caption{Comparison betwen MoCLR ImageNet pretrained network and VITO on natural distribution shifts. Accuracies are reported on different subsets ImageNet subject to different distortions. All datasets and evaluation follow \citet{taori2020measuring}. }
\label{tab:robust}
\vspace{-1.em}
\end{table}
